Mechanism Design for Team Formation

Team formation is a core problem in AI. Remarkably, little prior work has addressed the problem of mechanism design for team formation, accounting for the need to elicit agents' preferences over potential teammates. Coalition formation in the related hedonic games has received much attention, but only from the perspective of coalition stability, with little emphasis on the mechanism design objectives of true preference elicitation, social welfare, and equity. We present the first formal mechanism design framework for team formation, building on recent combinatorial matching market design literature. We exhibit four mechanisms for this problem, two novel, two simple extensions of known mechanisms from other domains. Two of these (one new, one known) have desirable theoretical properties. However, we use extensive experiments to show our second novel mechanism, despite having no theoretical guarantees, empirically achieves good incentive compatibility, welfare, and fairness.

==> preliminaries.tex <==
\section{Preliminaries}

\subsection{Hedonic Games}

Our point of departure is the formalism of \emph{hedonic games}.
We define a \emph{hedonic game} as a tuple $(N, \succ)$, where $N$ is the set of players, and $\succ$ is a vector containing each player's preference order over sets of other players that it could be teamed up with. 
%$\succ_i$ is the preference order of player $i$ over sets of other players, which induces a total order on player sets $S$, with $S \subset N_{-i}$. 
%The task is to partition the players in $N$ into a coalition structure, where each player is in exactly one coalition.

We assume that player preferences are \emph{additively separable}~\cite{aziz2011stable}, which means that there exists an assignment of values $u_i(j)$ for all players $i$ and their potential teammates $j$, so that $i$'s total utility of a subset of others $S$ is $\sum_{j \in S} u_i(j)$ (which induces a corresponding preference ordering over subsets of possible teammates).
In addition, we assume that $u_i(j) \ge 0$ for all $i,j$.
%Under \emph{additively separable preferences} with non-negative values, for each player $i$, that player's preference order $\succ_i$ must be additive separable. This means that there exists some mapping from other players to real values, $f: N_{-i} \rightarrow \mathbb{R+}$, such that, for any two sets $S$, $S' \subset N_{-i}$, player $i$ prefers the set with greater total value $u_i(j)$ over its players $j$:

%\begin{align*}
%S \succ_i S' \iff \sum_{j \in S} u_i(j) > \sum_{j' in S'} u_i(j')
%\end{align*}

%Additively separable hedonic games (ASHGs) can be viewed as a form of graph coloring game, where the players are nodes in a complete directed graph, the edge weights correspond to players' values for each other, and the goal is to color nodes to produce same-color cliques with high edge weights \cite{aziz2011stable}.

\subsection{Mechanism Design Problem}

Of typical interest in the extensive literature on hedonic games is coalition stability.
Our goal is distinct: we take as input player preferences over teams (that is, over others that they could be teamed up with), which we assume to be additive with positive values, and output a partition of the players into teams.
We assume that it is subsequently difficult for players to alter team membership.
Our primary challenge, therefore, is to encourage players to report their preferences honestly, and form teams that are fair and yield good teammate matchings; all three notions shall be made precise presently.
%Assuming that these are reported honestly to the center, these form a hedonic game.
%The task is to partition the players in $N$ into a coalition structure, where each player is in exactly one coalition.
Note that in this construction we assume that no money can change hands.

First, we observe that in our setup all players always prefer to be put on a single team (since values for all potential teammates are positive).
In reality, many team formation problems have hard constraints on team sizes (or, equivalently, on the number of teams), particularly when a diversity of tasks need to be accomplished.
For example, project teams (especially in courses) usually have an upper bound on size.
We capture this by introducing team size constraints; formally, the size of any team must be in the interval $[\underline{k},\overline{k}]$, with $\underline{k} \ge 1$, $\overline{k} \le |N|$, and $\underline{k} \le \overline{k}$.
%We extend additively separable hedonic games (henceforth, ASHGs) with \emph{coalition size constraints}. It is natural to consider that in real-world team formation problems, it may not be practical to form the grand coalition, with all agents on one team, even though this is preferred by the agents in an ASHG with non-negative values. We let $\underline{k} \geq 1$ be the minimum allowed team size and $\overline{k} \leq \|N\|$ be the maximum allowed team size. Additionally, we require that $\underline{k} \leq \overline{k}$. 
For example, if a classroom with $25$ students must be divided into $6$ approximately equal-size teams, we could have $\underline{k} = 4$ and $\overline{k} = 5$. 
We assume throughout that the specific values of $\underline{k}$ and $\overline{k}$ admit a feasible allocation (this is not always the case).

In contrast with a typical approach to mechanism design, which involves maximizing a single objective such as social welfare or designer revenue, subject to incentive compatibility (and possibly other) constraints, we pick up a thread from the matching market design literature (which our setting resembles), which tends to focus on a collection of \emph{desirable properties} (see, e.g., \citeauthor{Budish12}~\shortcite{Budish12}).
Specifically, we consider three properties: incentive compatibility, social welfare, and fairness.
Given the fact that all three cannot be achieved simultaneously in our setting, we will focus on the extent each can be achieved through specific mechanisms.

\paragraph{Incentive Compatibility}

Incentive compatibility is about ensuring that there is no incentive for any agent to misreport their preferences.
We consider two forms of incentive compatibility: \emph{strategyproofness}, which is incentive compatibility in dominant strategies, and \emph{ex post}, which ensures that truthful reporting is an equilibrium for any collection of player preferences.
The former will be considered in theoretical analysis, while the latter will be the focus of empirical incentive assessment.
In particular, our theory will focus on \emph{strategyproofness-in-the-large}~\cite{budish2011combinatorial}, defined as follows.
Consider a market where each agent has been replaced with ``a measure-one continuum of replicas'' of itself, such that each individual agent has zero measure and all agents are ``price takers.'' A mechanism is strategyproof-in-the-large if, in such a market, it is a dominant strategy for each agent to reveal its true preferences. An example of a mechanism that is not strategyproof-in-the-large is the Harvard Business School draft considered below, in which an agent may benefit from misreporting its preferences, regardless of its own measure relative to the market size \cite{budish2010multi}.
In empirical analysis, in contrast, we measure the \emph{regret of truthful reporting}, which is the most any agent can gain ex post by misreporting preferences when all others are truthful.

%Our criterion for incentivizing honest reporting is \emph{strategyproofness}.
%An allocation mechanism is \emph{strategyproof} if it is a dominant strategy for each agent to reveal its true preferences. In other words, if a mechanism is strategyproof, then no agent can increase its expected payoff by misreporting preferences, no matter what the other agents do.

%One measure of the incentive to lie is the \emph{regret of truthful reporting}. This measure is similar to the game theoretic \emph{regret} of a strategy profile, which is the maximum over agents of the maximum over alternative strategies for the agent, of the expected increase in payoff from unilaterally deviating to that strategy. The regret of truthful reporting is the maximum any agent can gain in expected payoff by misreporting its preferences, while all other agents reveal their true preferences.

%Budish proposes an approximate form of strategyproofness, called \emph{strategyproof-in-the-large} \cite{budish2011combinatorial}. Consider a market where each agent has been replaced with ``a measure-one continuum of replicas'' of itself, such that each individual agent has zero measure and all agents are ``price takers.'' A mechanism is strategyproof-in-the-large if, in such a market, it is a dominant strategy for each agent to reveal its true preferences. An example of a mechanism that is not strategyproof-in-the-large is the HBS draft, in which an agent may benefit from misreporting its preferences, regardless of its own measure relative to the market size \cite{budish2010multi}.

\paragraph{Social Welfare}

As in traditional mechanism design, we consider social welfare as one of our primary design criteria.
Social welfare is just the sum of player utilities achieved by a specific partition of players into teams.
Formally, if $\mathcal{P}$ is a partition of players, social welfare is defined as $SW(\mathcal{P}) = \sum_{S \in \mathcal{P}} \sum_{i,j \in S} u_i(j)$.

\paragraph{Fairness}

We consider a few measures of fairness in an allocation. An allocation is \emph{envy-free} if each agent weakly prefers its own allocation to that of any other agent. An allocation is \emph{proportional} if each agent's utility is at least as great as the total utility of all goods to that agent, divided by the number of teams that are formed. An allocation satisfies the \emph{maximin share guarantee} if for each agent, the agent weakly prefers its allocation to its \emph{maximin share}. A maximin share for an agent is the agent's least preferred bundle in a \emph{maximin split} for the agent, which is a partition of all goods into one bundle per agent that maximizes the utility of the least valuable bundle. Note that envy-freeness implies proportionality, and proportionality implies maximin shares \cite{procaccia2014fair}.

For hedonic games, we introduce a modified version of the maximin share guarantee, the \emph{maximin share guarantee for hedonic games}. A coalition structure in a hedonic game provides maximin shares for hedonic games, if each agent weakly prefers its bundle of other agents to its maximin share. Given $(N, \succ_i, \underline{k}, \overline{k})$, consider all partitions of the agents $N$ with coalition sizes in $[\underline{k}, \overline{k}]$. A maximin split for agent $i$ is any such partition that maximizes the value for $i$ of the least preferred coalition containing $i$, which would result from swapping $i$ with some agent $j$, where $j$ may equal $i$. A maximin share is the least preferred coalition in a maximin split. This definition of the maximin share guarantee preserves a useful property of the guarantee for multi-unit assignment, which is that an agent may be assigned one of $|N|$ bundles from its maximin split.

The maximin share guarantee for ASHGs with non-negative values is trivially satisfiable for $\overline{k} = |N|$: If the grand coalition is assigned, every agent's payoff is maximized, so envy-freeness is achieved. The maximin share guarantee for ASHGs with non-negative values is also trivially satisfiable for $\overline{k} = 2$. In the maximin split for an agent with $\overline{k} = 2$, all agents are grouped in pairs (assuming $|N|$ is even), and the agent's maximin share is the pair with its least favorite other agent. Thus, any grouping of the agents into pairs satisfies the maximin share guarantee.

\smallskip
\textbf{Proposition 1.} \emph{For some ASHGs with non-negative values, $\overline{k} \geq 3$, and $\overline{k} < |N|$, the maximin share guarantee for hedonic games is not satisfiable.}

\smallskip
\noindent
\emph{Example.} Consider a hedonic game with $6$ agents, $\{A, B, C, D, E, F\}$, $\underline{k} = 3$, $\overline{k} = 3$, so that two equal-size coalitions must be formed. The agents' additive separable preferences are encoded in Table 1.

\smallskip
\noindent
\begin{tabular}{ c | c c c c c c c }
     & $A$ & $B$ & $C$ & $D$ & $E$ & $F$ \\
  \hline
  $A$ & x & 1 & 0 & 2 & 3 & 2 \\
  $B$ & 2 & x & 1 & 0 & 3 & 2 \\
  $C$ & 2 & 2 & x & 1 & 0 & 3 \\
  $D$ & 1 & 2 & 2 & x & 2 & 1 \\
  $E$ & 0 & 2 & 3  & 1 & x & 2 \\
  $F$ & 2 & 1 & 2 & 2 & 1 & x \\
\end{tabular} \\

\smallskip
\noindent
\textbf{Table 1.} Value of each agent to each other agent. Each row shows the value of other agents to a single evaluating agent.

\smallskip
It is easy to see that in the game described above, each agent's maximin share for hedonic games has value $3$. Furthermore, any of the $10$ possible partitions of the agents into two equal-size groups leaves some agent with a coalition value of $2$ or less. Therefore, no partition for this game provides every agent with a maximin share. In consequence, no partition for this game is proportional or envy-free either. \qed

==> theory.tex <==
\section{Theory}

\subsection{Feasibility of Coalition Size Constraints}
Some tuples $(N, \underline{k}, \overline{k})$ are not feasible, meaning that it is not possible to divide $\|N\|$ players into coalitions with sizes in $[\underline{k}, \overline{k}]$. Recall that we require by definition $1 \leq \underline{k} \leq \overline{k} \leq \|N\|$. For a minimal example, it is not possible to divide $3$ players into coalitions with $\underline{k} = 2$, $\overline{k} = 2$.

\smallskip
\noindent
\textbf{Observation 1.} \emph{A tuple $(N, \underline{k}, \overline{k})$ is feasible if and only if: $\underline{k}$ divides $N$, $\overline{k}$ divides $N$, or $(N \setminus \underline{k}) > (N \setminus \overline{k})$, where $\setminus$ signifies integer division.}

For the rest of this paper, we assume that we are working with ASHGs with non-negative values and feasible coalition size constraints.

\subsection{Maximin Share Guarantee}
The maximin share guarantee for ASHGs with non-negative values is trivially satisfiable for $\overline{k} = \|N\|$: If the grand coalition is assigned, every agent's payoff is maximized, so envy-freeness is achieved. The maximin share guarantee for ASHGs with non-negative values is also trivially satisfiable for $\overline{k} = 2$. In the maximin split for an agent with $\overline{k} = 2$, all agents are grouped in pairs (assuming $\|N\|$ is even), and the agent's maximin share is the pair with its least favorite other agent. Thus, any grouping of the agents into pairs satisfies the maximin share guarantee.

\smallskip
\textbf{Proposition 1.} \emph{For some ASHGs with non-negative values, $\overline{k} \geq 3$, and $\overline{k} < \|N\|$, the maximin share guarantee for hedonic games is not satisfiable.}

\smallskip
\noindent
\emph{Example.} Consider a hedonic game with $6$ agents, $\{A, B, C, D, E, F\}$, $\underline{k} = 3$, $\overline{k} = 3$, so that two equal-size coalitions must be formed. The agents' additive separable preferences are encoded in Table 1.

\smallskip
\noindent
\begin{tabular}{ c | c c c c c c c }
     & $A$ & $B$ & $C$ & $D$ & $E$ & $F$ \\
  \hline
  $A$ & x & 1 & 0 & 2 & 3 & 2 \\
  $B$ & 2 & x & 1 & 0 & 3 & 2 \\
  $C$ & 2 & 2 & x & 1 & 0 & 3 \\
  $D$ & 1 & 2 & 2 & x & 2 & 1 \\
  $E$ & 0 & 2 & 3  & 1 & x & 2 \\
  $F$ & 2 & 1 & 2 & 2 & 1 & x \\
\end{tabular} \\

\smallskip
\noindent
\textbf{Table 1.} Value of each agent to each other agent. Each row shows the value of other agents to a single evaluating agent.

\smallskip
It is easy to see that in the game described above, each agent's maximin share for hedonic games has value $3$. Furthermore, any of the $10$ possible partitions of the agents into two equal-size groups leaves some agent with a coalition value of $2$ or less. Therefore, no partition for this game provides every agent with a maximin share. In consequence, no partition for this game is proportional or envy-free either. \qed

\subsection{Price-Based Mechanisms for Team Formation}

A price-based mechanism for team formation, such as A-CEEI-TF, assigns a price $p_i \in \mathbb{R+}$ and a budget $b_i \in \mathbb{R+}$ to each agent. An agent can demand only those bundles of other agents whose total price is less than the agent's budget. Note that an agent is not required to pay its own price.

Each agent reports to the clearinghouse the additive separable utility it gains from each other agent. The clearinghouse uses these reports to derive which affordable bundle of other agents each agent demands, given each agent's budget and price. The total utility for an agent $i$ of a bundle of other agents of size in $[\underline{k} - 1, \overline{k} - 1]$, is the sum of the utilities for agent $i$ of the agents in that bundle. The utility of any illegally-sized bundle of agents is defined as $0$. The clearinghouse will provisionally assign agent $i$ the bundle of highest utility for $i$ that it can afford, or the empty bundle if it cannot afford any bundle of legal size.

\smallskip
\noindent
\textbf{Proposition 2.} \emph{For some ASHGs with non-negative values, $\underline{k} > 1$, and $\overline{k} < \|N\|$, no price vector $p$ and budget vector $b$ exist that induce exact market clearing.}

We define \emph{exact market clearing for hedonic games} to mean that when each agent is allocated its favorite bundle of other agents that is affordable:

\begin{itemize}
\item Each agent is assigned to a coalition with size in $[\underline{k}, \overline{k}]$, including itself in the coalition size.
\item For any two distinct agents $i$ and $j$, $i$ demands $j$ if and only if $j$ demands $i$.
\end{itemize}

This result marks a distinction from the course allocation problem, where with sufficiently unequal budgets, some price vector must exist that induces exact market clearing \cite{budish2011combinatorial}.

\noindent
\emph{Example.} Consider a hedonic game with $4$ agents, $\{A, B, C, D\}$, with $\underline{k} = 2$ and $\overline{k} = 2$. The agents' additive separable preferences are encoded in Table 2.

\smallskip
\begin{tabular}{ c | c c c c }
     & $A$ & $B$ & $C$ & $D$ \\
  \hline
  $A$ & x & 2 & 1 & 0 \\
  $B$ & 0 & x & 2 & 1 \\
  $C$ & 1 & 0 & x & 2 \\
  $D$ & 2 & 1 & 0 & x \\
\end{tabular} \\

\smallskip
\noindent
\textbf{Table 2.} Value of each agent to each other agent. Each row shows the value of other agents to a single evaluating agent.

\smallskip
In the example, only two allocations must be considered, due to symmetry: $\{\{A, B\}, \{C, D\}\}$ and $\{\{A, C\}, \{B, D\}\}$.

In order for the market to clear as $\{\{A, B\}, \{C, D\}\}$, each agent must be able to afford its assigned partner, and each agent must not be able to afford any other agent that it prefers. If we assume the market clears in this way, the resulting inferences produce an impossible conclusion:

\begin{align*}
p_A \leq b_B < p_C \leq b_D < p_A 
\end{align*}

A similar conclusion can be drawn from the other allocation, $\{\{A, C\}, \{B, D\}\}$. We find that no $(b, p)$ induces exact market clearing for this game, no matter how unequal the agents' budgets in $b$ are. \qed

\smallskip
We define a notion of \emph{relaxed market clearing}, which we will use in our search for approximately market-clearing prices. This form of market clearing allows a good on the market to be under-demanded if and only if its price is $0$. We adapt this relaxed form of market clearing from Budish \cite{budish2011combinatorial}. In relaxed market clearing:

\begin{itemize}
\item Each agent is assigned to a coalition with size in $[\underline{k}, \overline{k}]$, including itself in the coalition size, unless the agent has price $0$, in which case it may alternatively be assigned the team containing only itself.
\item For any two distinct agents $i$ and $j$, $i$ demands $j$ if and only if $j$ demands $i$.
\end{itemize}

\subsection{Approximate Competitive Equilibrium from Equal Incomes for Team Formation}

\smallskip
\noindent
\textbf{Proposition 3.} \emph{The function $f(\cdot)$ is a viable price update function for A-CEEI-TF, because: (a) for any fixed point $\tilde{p} \in \mathcal{\tilde{P}}$, $p = t(\tilde{p})$ must induce relaxed market clearing, and (b) the auxiliary price space $\mathcal{\tilde{P}}$ is closed under $f(\cdot)$.}

\smallskip
\noindent
\emph{Proof.} First, we show that auxiliary price space $\mathcal{\tilde{P}}$ is closed under $f(\cdot)$. The range of $z(p)_j$ for $p \in \mathcal{P}$ is $[-1, (\|N'\| - 1)(1 + \epsilon)]$. Thus, assuming $\epsilon$ is small, $|z(p)_j / \|N'\|| < 1$. Therefore, it is easy to see that auxiliary price space $[-1, 1 + \bar{b}]^{\|N'\|}$ is closed under $f(\cdot)$.

Next, we show that if $\tilde{p} \in \mathcal{\tilde{P}}$ is a fixed point of $f(\cdot)$, then $p = t(\tilde{p})$ must induce relaxed market clearing.

Each agent price $p_j$ in $p = t(\tilde{p})$ must either equal $0$, equal $\bar{b}$, or be in $(0, \bar{b})$.

If $p_j = \bar{b}$, then no agent can afford to demand agent $j$, so $UND_j = 1$ and $IURQ_j = 0$, implying that $z(p)_j$ is negative, so $p_j$ cannot be a fixed point. If $p_j$ has been truncated by $t(\cdot)$, this would reduce it, and $z(\cdot)$ further reduces it.

If $p_j = 0$, then if there is $IURQ_j > 0$ and $UND_j = 0$, the net effect of $z(p)_j$ is to increase $p_j$, and if $p_j$ has been truncated, then that would have increased $p_j$ also; so with or without truncation, $p_j$ would not be a fixed point if it had positive $IURQ$ but not $UND$. If $p_j = 0$ and $IURQ = 0$, then under-demand for $j$ is allowed because the price of $j$ is zero, so this does not violate relaxed market clearing. $IURQ_j$ and $UND_j$ cannot both be positive, because if there is incoming demand, there is no under-demand by definition.

If $p_j \in (0, \bar{b}$), and $p_j$ is part of a fixed point $p$, then $UND_j = 0$ and $IURQ_j = 0$, because by definition, they cannot both be positive at once. \qed

\smallskip
\noindent
\textbf{Proposition 4.} \emph{There exists a point $p^*$ in price space $\mathcal{P}$, for which a convex combination of the error terms $z(p')$ induced by some set of prices near $p^*$ equals the zero vector, as in relaxed market clearing.}

\smallskip
\noindent
\emph{Proof sketch.} The proposition can be proved through a straightforward adaptation of the proof of Theorem 1 in Budish \cite{budish2011combinatorial}. First we note that any fixed point of $f(\cdot)$ induces relaxed market clearing. Furthermore, the price space $\mathcal{\tilde{P}}$ is compact, convex, and closed under $f(\cdot)$. We introduce a function $F(\tilde{p})$ that takes the convex hull of all values $f(\tilde{p}')$, for $\tilde{p}'$ approaching in the limit but not equal to $\tilde{p}$. 

Lemma 2.4 of Cromme and Diener is useful here \cite{cromme1991fixed}. Take any space $\mathcal{X}$ that is a non-empty, compact, convex subset of $\mathbb{R}^d$, and any function $f: \mathcal{X} \rightarrow \mathcal{X}$, such that $\mathcal{X}$ is closed under $f$. Define $H_f: \mathcal{X} \rightarrow S$, $S \subset \mathcal{X}$, to be the function that takes any $x$ in $\mathcal{X}$ and yields the set:

\begin{align*}
\{y \in \mathcal{X} | \exists \textrm{ a sequence } x_i \rightarrow x, x_i \neq x : f(x_i) \rightarrow y \}
\end{align*}

Lemma 2.4 of Cromme and Diener states that for any such function $f$, there exists a point $x^* \in \mathcal{X}$ such that $x^*$ is in the convex hull of $H_f(x^*)$.

We can apply Cromme and Diener's result to $F(\cdot)$, because the auxiliary price space $\mathcal{\tilde{P}}$ is non-empty, compact, convex, and closed under $f(\cdot)$, and $F(\cdot)$ is defined as the convex hull of Cromme and Diener's $H_f$. Therefore, as shown in Cromme and Diener, Kakutani's fixed point theorem implies that $F(\cdot)$ has a fixed point $\tilde{p}^*\in \mathcal{\tilde{P}}$. Thus, a convex combination of the error terms $z(p')$ near $t(\tilde{p}^*)$ yields relaxed market clearing. \qed

\smallskip
As in the work of Budish, our fixed point result suggests that for prices $p'$ in the neighborhood of the truncation of a fixed point $\tilde{p}^*$ of the price update function, induced market clearing error will be low. Therefore, we will likely be able to find price vectors that yield low market clearing error by iteratively applying $f(\cdot)$ to its own output, until an apparent fixed point is approached.

\smallskip
\noindent
\textbf{Proposition 5.} \emph{A-CEEI-TF is strategyproof-in-the-large.}

\smallskip
\noindent
\emph{Proof sketch.} Any individual agent in the continuum economy, being zero-measure, has no influence on the approximate equilibrium price vector arrived at by update function $f(\cdot)$, at any iteration of the A-CEEI-TF mechanism. Therefore, the only effect the agent can have on the outcome is that, if the agent is randomly selected to choose its favorite affordable bundle of free agents that leaves a feasible subproblem, the agent's reported preferences determine which bundle the agent is assigned. Thus, it is a dominant strategy for the agent to report its true preferences, so that in this case the agent will be assigned its most preferred allowable team. \qed

%\subsection{Other Mechanisms for Team Formation}

%We use a few baseline mechanisms for comparison to our novel mechanisms, A-CEEI-TF and the OPOP draft.

%Each of these mechanisms uses the following method to keep team sizes balanced. Given a number of players $\|N\|$ and maximum team size $k$, we first select the most similar feasible $\underline{k}$ and $\overline{k}$, where $\overline{k} \leq k$. Note that $\overline{k} \leq \underline{k} + 1$. Then we generate the list of team sizes that is non-decreasing, contains as many values of size $\overline{k}$ as possible, and sums to $\|N\|$. Let the length of this list, indicating the number of teams to be formed, be called $T$. This list determines the team sizes to be formed in each mechanism below.

%\begin{itemize}
%\item \textbf{Random allocation.} Given a list of team sizes as described above, players are uniformly randomly assigned to teams. Random allocation is strategyproof, but not Pareto efficient.
%\item \textbf{Random serial dictatorship.} Players are randomly ordered. The next unchosen player in order selects its favorite other unchosen players, up to the next team size in the list. Repeat until all players are assigned. Random serial dictatorship is strategyproof. If the mechanism is defined such that the current captain may choose a team of any legal size that leaves a feasible subproblem, it is Pareto efficient. As defined above, it may not be Pareto efficient, but expected fairness is improved.
%\item \textbf{Maximize social welfare.} Assign players to $T$ teams of size in $[\underline{k}, \overline{k}]$, so as to maximize the total over players of the total value of the player's teammates. Maximize social welfare is not strategyproof, but it is Pareto efficient.
%\item \textbf{HBS draft for team formation.} Players are randomly ordered. Given the list of team sizes, the first $T$ players are assigned to be captains of the respective teams. Then iterate over team captains, first in player order, then in reverse player order, alternating. The current team captain selects its most preferred remaining player to join its team, based on its reported preferences. The HBS draft is not strategyproof or Pareto efficient.
%\item \textbf{One-Player-One-Pick draft.} Players are randomly ordered. Given the list of team sizes, the first $T$ players are assigned to be captains of the respective teams. Then iterate over the complete player list. If the next player is a team captain, it selects its favorite unassigned agent to join its team. If the next player is unassigned, it will be assigned to join its favorite incomplete team (as defined below). If the next player has been assigned to a team that is incomplete, it selects its favorite unassigned agent to join its team. Otherwise the player does nothing. The OPOP draft is not strategyproof or Pareto efficient.
%\end{itemize}

%In the OPOP draft, we select the ``favorite'' incomplete team for an unassigned player to join as follows. Let $S$ be an incomplete team with $v_S$ vacancies. Let the mean value to player $i$ of the other unassigned players be $\mu_i$. Incomplete team $S$ has expected value to unassigned agent $i$:

%\begin{align*}
%\sum_{j \in S} u_i(j) + (v_S - 1) \mu_i
%\end{align*}

%In words, player $i$ expects team $S$ to be worth the sum of the values of its current agents, plus the mean value of other unassigned agents, times the number of vacancies left minus $1$ for the space claimed by $i$ itself. An unassigned player in the OPOP draft will be assigned to the team of maximum expected value, based on its reported preferences.

\smallskip
\noindent
\textbf{Observation 2.} \emph{The One-Player-One-Pick draft is not strategyproof.}

 It may be less obvious that the OPOP draft is not strategyproof, compared to the HBS draft, because in the OPOP draft, each player makes at most one selection. In the HBS draft, a player can benefit from under-reporting its value for unpopular items, because such items are likely to remain available after multiple rounds of the draft, while less valuable but more popular items will likely be taken in an early round. In the OPOP draft, no such incentive to lie exists, because each player makes at most one selection.

Note that the HBS draft and OPOP draft are strategyproof for hedonic games with $\overline{k} = 2$, because in such cases these mechanisms are equivalent to random serial dictatorship, as each team captain chooses only one other player to join it.

\smallskip
\noindent
\emph{Example.} Consider a minimal-size example of an ASHG with non-negative values, where the OPOP draft is not strategyproof. Let $N = \{A, B, C, D, E, F\}$, $\underline{k} = 3$, and $\overline{k} = 3$. The players' additive separable values to each other are encoded in the table below.

\smallskip
\begin{tabular}{ c | c c c c c c c }
     & $A$ & $B$ & $C$ & $D$ & $E$ & $F$ \\
  \hline
  $A$ & x & 5.0 & 4.9 & 7.0 & 0.2 & 0.0 \\
  $A'$ & x & 5.0 & 6.0 & 7.0 & 0.2 & 0.0 \\
  $B$ & 0.0 & x & 1.1 & 1.6 & 1.2 & 1.3 \\
  $C$ & 0.0 & 1.1 & x & 1.6 & 1.2 & 1.3 \\
  $D$ & 0.0 & 1.1 & 1.6 & x & 1.2 & 1.3 \\
  $E$ & 0.0 & 1.1 & 1.6  & 1.2 & x & 1.3 \\
  $F$ & 0.0 & 1.1 & 1.6 & 1.2 & 1.3 & x \\
\end{tabular} \\

\smallskip
\noindent
\textbf{Table 3.} Value of each agent to each other agent. Each row shows the value of other agents to a single evaluating agent. Row $A'$ shows the false report of agent $A$.

\smallskip
The OPOP draft is a randomized allocation mechanism, which works by uniformly randomly choosing a permutation of the players, then acting deterministically based on that order. Strategyproofness for a randomized mechanism means that a player's expected payoff is maximized by truthful reporting, regardless of other players' actions. To show that the OPOP draft is not strategyproof, it suffices to show that player $A$ gains in expected payoff, based on the true preferences in row $A$ of the table, by misreporting its preferences as in row $A'$ in the table, if other players report their preferences as displayed in the table.

The example game has $6$ players, so there are $6! = 720$ permutations, and $720$ equally likely outcomes from the OPOP draft, some of which are identical in their allocations. It turns out that the payoff for player $A$ is better when reporting $A'$ instead of $A$ for $18$ of $720$ permutations, and worse in $6$ others. Specifically, player $A$ performs better by lying if and only if the order of the first three players to choose is $(ADB)$, $(ADE)$, or $(ADF)$. Player $A$ does worse by reporting $A'$ if and only if the order of the first three players is $(ADC)$. After factoring in the value of the resulting allocations to player $A$, it results that the expected value of defecting to $A'$ is $0.08$ utils per game. Thus, the OPOP draft is not strategyproof. \qed
